The tangential cone condition for some coefficient identification model problems in parabolic PDEs

The tangential condition was introduced in [Hanke et al., 95] as a sufficient condition for convergence of the Landweber iteration for solving ill-posed problems. In this paper we present a series of time dependent benchmark inverse problems for which we can verify this condition.

==> sec1dot3.tex <==
\subsection{An inverse source problem with a quadratic first order nonlinearity}
In this subsection, we are interested in the problem of identifying the space-dependent source term $\theta$ from observation of the state $u$
\begin{flalign} 
&\qquad\qquad\qquad\dot{u}-\Delta u - |\nabla u|^2=\theta \qquad (t,x) \in (0,T)\times \Omega& \label{log-problem-1}\\
&\qquad\qquad\qquad u_{|\partial\Omega}=0 \qquad\qquad\qquad\hphantom{hh} t \in (0,T)&	\label{log-problem-2}\\
&\qquad\qquad\qquad u(0)=u_0 \qquad\qquad\qquad\hphantom{h} x \in \Omega &	\label{log-problem-3}
\end{flalign}
on the function spaces
\begin{align} \label{log-space}
 \calX=L^p(\Omega),  \quad\qquad Y=L^q(\Omega),  \quad\qquad  V=W=H^2(\Omega)\cap H_0^1(\Omega). \qquad
\end{align} 
This sort of PDE with a quadratic nonlinearity in $\nabla u$ arises, e.g., in stochastic optimal control theory \cite[Chapter 3.8]{FlemingSoner}.\\

By the transformation $\utransf:=e^u$, the initial-value problem (\ref{log-problem-1})--(\ref{log-problem-3}) can be converted into the c-problem type in Section \ref{c-problem}
\begin{flalign} 
&\qquad\qquad\qquad\dot{\utransf}-\Delta \utransf +\theta\utransf=0 \qquad (t,x) \in (0,T)\times \Omega& \label{transf-log-problem-1}\\
&\qquad\qquad\qquad \utransf_{|\partial\Omega}=1 \qquad\qquad\qquad\hphantom{hh} t \in (0,T)&	\label{transf-log-problem-2}\\
&\qquad\qquad\qquad \utransf(0)=\utransf_0 \qquad\qquad\qquad\hphantom{h} x \in \Omega &	\label{transf-log-problem-3}
\end{flalign}
with $\utransf_0=e^{u_0}$.
Thus, in principle it is covered by the analysis from the previous section, as long as additionally positivity of $\utransf$ can be established. 
So the purpose of this section is to investigate whether we can allow for different function spaces $X,Y$ by directly considering (\ref{log-problem-1})--(\ref{log-problem-3}) instead of (\ref{transf-log-problem-1})--(\ref{transf-log-problem-3}). 

%\textcolor{blue}{(Note: AAO-TCC for log-problem in Hilbert setting requires $(V,W)=(H^2,H^2)$ or $(H^{>2.5},H^1)$)\\}

We show that $f$ verifies the hypothesis proposed for the tangential cone condition in the reduced setting


\begin{enumerate}[label=(R\arabic*)]
\item \textit{Local Lipschitz continuity of $f$}
\begin{align*}
\|-|\nabla\tilde{u}|^2+|\nabla u|^2 - \tilde{\theta}+\theta\|_{W^*}
&= \sup_{\|w\|_W \leq 1} \int_\Omega \left(\nabla(u-\tilde{u})\cdot\nabla(u+\tilde{u})- \tilde{\theta} + \theta \right)w dx\\
&\leq C_{W\rightarrow L^{\bar{p}}}\left(\|(\nabla(u-\tilde{u})\cdot\nabla(u+\tilde{u})\|_{L^{\frac{\bar{p}}{\bar{p}-1}}} + \|\theta-\tilde{\theta}\|_{L^{\frac{\bar{p}}{\bar{p}-1}}} \right)\\
&\leq C_{W\rightarrow L^{\bar{p}}}\left(\|\nabla(u-\tilde{u})\|_{L^{\frac{2\bar{p}}{\bar{p}-1}}}\|\nabla(u+\tilde{u})\|_{L^{\frac{2\bar{p}}{\bar{p}-1}}} + \|\theta-\tilde{\theta}\|_{L^{\frac{\bar{p}}{\bar{p}-1}}} \right)\\
&\leq C_{W\rightarrow L^{\bar{p}}}\left( C^2_{V\rightarrow W^{1,{\frac{2\bar{p}}{\bar{p}-1}}}}\|u-\tilde{u}\|_V\|u+\tilde{u}\|_V + C_{\calX\rightarrow L^{\frac{\bar{p}}{\bar{p}-1}}} \|\theta-\tilde{\theta} \|_\calX \right).
\end{align*}
Hence we can chose $L(M)=C_{W\rightarrow L^{\bar{p}}}\left(C^2_{V\rightarrow W^{1,{\frac{2\bar{p}}{\bar{p}-1}}}} (\|u\|_V+\|\tilde{u}\|_V ) + C_{\calX\rightarrow L^{\frac{\bar{p}}{\bar{p}-1}}}\right) +1$, under the conditions
\begin{equation} \label{log-cond-1}
\begin{split}
&V=H^2(\Omega)\cap H_0^1(\Omega) \hookrightarrow W^{1,{\frac{2\bar{p}}{\bar{p}-1}}}(\Omega)\mbox{ i.e., } \quad 1-\frac{d}{2}\geq -\frac{d(\bar{p}-1)}{2\bar{p}} \qquad\qquad\quad\\
&\calX=L^p(\Omega) \hookrightarrow L^{\frac{\bar{p}}{\bar{p}-1}}(\Omega)\mbox{ i.e., }\quad p \geq \frac{\bar{p}}{\bar{p}-1}. 
\end{split}
\end{equation}


%\textcolor{blue}{(****** R2 new. update on 22Sep)}

\item Well-definedness and boundedness of parameter-to-state map\medbreak

We argue unique existence of the solution to (\ref{log-problem-1})--(\ref{log-problem-3}) via the transformed problem 
(\ref{transf-log-problem-1})--(\ref{transf-log-problem-3}) for $\utransf=e^u$.


\quad To begin, by a similar argument to (\ref{c-contraction}) with the elliptic operator $A=-\Delta+\theta, \theta\in L^p(\Omega)$ in place of the parabolic operator, we show that the corresponding elliptic problem admits a unique solution in $H^2(\Omega)\cap H_0^1(\Omega)$ if the index $p$ satisfies (\ref{c-cond-3}). Employing next the semigroup theory in \cite[Section 7.4.3, Theorem 5]{Evans} or \cite[Chapter 7, Corollary 2.6]{Pazy} with assuming that $\utransf_0\in D(A)=H^2(\Omega)\cap H_0^1(\Omega)$ implies unique existence of a solution $\utransf\in C^1(0,T;H^2(\Omega))$ to \eqref{transf-log-problem-1}--\eqref{transf-log-problem-3}.
  
\quad Let $\utransf,\hat{\utransf}$ respectively solve \eqref{transf-log-problem-1}--\eqref{transf-log-problem-3} associated with the coefficients $\theta\in \calX, \hat{\theta}\in L^\infty(\Omega)$ with the same boundary and initial data, then $v=\utransf-\hat{\utransf}$ solves 
\begin{flalign*} 
&\qquad\qquad\qquad\dot{v}(t)-\Delta v(t) + \hat{\theta}v(t) = (\hat{\theta}-\theta)\utransf(t) \qquad t \in (0,T) &\\
&\qquad\qquad\qquad v(0)=0. &	
\end{flalign*}
Owing to the regularity from \cite[Section 7.1.3, Theorem 5]{Evans} and estimating similarly to (\ref{c-contraction}), we obtain
\begin{align} \label{log-positive-estimate-1}
\|\utransf-\hat{\utransf}\|_{L^\infty(0,T;H^2(\Omega))} 
\leq C^{\hat{\theta}}\|(\hat{\theta}-\theta)\utransf\|_{H^1(0,T;L^2(\Omega))} 
\leq C\|\hat{\theta}-\theta\|_\calX\|\utransf\|_{H^1(0,T;H^2(\Omega))}
\end{align}
\textcolor{blue}{with positive $\hat{\utransf}$ since $\hat{\theta}\in L^\infty(\Omega)$ and the constant $C$ depending only on $\theta^0, \rho$. Here we assume $\hat{\theta}=\theta^0\in L^\infty(\Omega)$ and $\rho$ is sufficiently small such that the right hand side is sufficiently small.} Then $\utransf\in L^\infty(0,T;H^2(\Omega))\subseteq L^\infty((0,T)\times\Omega)$ is close to $\hat{\utransf}$ and therefore positive as well. This assertion is valid if $0< \utransf_0=e^{u_0}\in H^2(\Omega)\cap H_0^1(\Omega)$, $0<\utransf|_{\delta\Omega}$, which is chosen as $\utransf|_{\delta\Omega}=1$ in this case (such that $\log(\utransf|_{\delta\Omega})=0$), and 
\begin{equation} \label{log-cond-2}
\begin{split}
&H^2(\Omega)\hookrightarrow L^{\frac{2p}{p-2}}(\Omega)\mbox{ i.e.,} \quad p\geq\frac{2\bar{p}}{\bar{p}-2} \quad\qquad\qquad\qquad\qquad\\
&V= H^2(\Omega)\hookrightarrow L^\infty(\Omega)\mbox{ i.e.,}\quad d\leq 3. 
\end{split}
\end{equation}

This leads to unique existence of the solution $u:=\log(\utransf)$ to the problem (\ref{log-problem-1})--(\ref{log-problem-3}), moreover  $0<\underline{c}\leq \utransf \in C^1(0,T;H^2(\Omega))$ allows $u=\log(\utransf) \in  C^1(0,T;H^2(\Omega)\cap H_0^1(\Omega))$.\\
\textcolor{blue}{
If $d=1, p\geq2$, no assumption on smallness of $\rho$ is required since
\begin{align} \label{log-positive-estimate-2}
\|\utransf-\hat{\utransf}\|_{L^\infty(0,T;H^1(\Omega))}
&\leq C^\theta\|(\hat{\theta}-\theta)\hat{\utransf}\|_{L^2(0,T;L^2(\Omega))}\leq C\|\hat{\theta}-\theta\|_\calX\|\hat{\utransf}\|_{L^2(0,T;H^2(\Omega))} 
\end{align}
due to the estimates \eqref{c-rho-1}--\eqref{c-regularity} in the c-problem. Here the constant $C$ depends only on $\theta^0, \rho$ as claimed in (\ref{c-regularity}). This and the fact $\overline{L^\infty(\Omega)}=L^p(\Omega)$ allow us to chose $\hat{\theta}\in L^\infty(\Omega)$ being sufficiently close to $\theta\in L^p(\Omega)$ to make the right hand side of (\ref{log-positive-estimate-2}) arbitrarily small without the need of smallness of $\rho$.\\
}
\quad We have observed that, with the same positive boundary and initial data, the solution to the c-problem $\utransf=\utransf(\theta)$ is bounded away from zero for all $\theta\in\calB^\calX_\rho(\theta^0)$. Besides, $S:\theta\mapsto \utransf$ is a bounded operator as proven in \ref{R2} of the c-problem. Consequently, $u=\log(\utransf)$ with $\Delta u=-\frac{|\nabla \utransf|^2}{\utransf^2}+\frac{\Delta \utransf}{\utransf}$ is uniformly bound in $L^2(0,T;H^2(\Omega)\cap H_0^1(\Omega))$ for all $\theta\in\calB^\calX_\rho(\theta^0)$  thus $S:\theta\mapsto u$ is a bounded operator on $\calB^\calX_\rho(\theta^0)$.

\color{blue}
Moreover, we can derive a uniform bound for $\utransf$ in $H^1(0,T;H^2(\Omega))$ with respect to $\theta$. From
\begin{align*}
(\dot{\utransf}-\dot{\hat{\utransf}}) - \Delta(\utransf-\hat{\utransf}) + (\theta-\hat{\theta})(\utransf-\hat{\utransf})=-\hat{\theta}(\utransf-\hat{\utransf})-(\theta-\hat{\theta})\hat{\utransf},
\end{align*}
by taking time derivative of both sides then test them with $-\Delta(\dot{\utransf}-\dot{\hat{\utransf}})$ we have
\begin{align*}
&\frac{1}{2}\frac{d}{dt}\|\nabla(\dot{\utransf}-\dot{\hat{\utransf}})\|^2_{L^2(\Omega)}+\|\Delta(\dot{\utransf}-\dot{\hat{\utransf}})\|^2_{L^2(\Omega)}\\
&\leq C_{H^2\hookrightarrow L^\infty}\|\theta-\hat{\theta}\|_{L^2(\Omega)}\|\Delta(\dot{\utransf}-\dot{\hat{\utransf}})\|^2_{L^2(\Omega)}
+\|\hat{\theta}\|_{L^\infty(\Omega)}\|\dot{\utransf}-\dot{\hat{\utransf}}\|_{L^2(\Omega)}\|\Delta(\dot{\utransf}-\dot{\hat{\utransf}})\|_{L^2(\Omega)}\\
&\qquad +C_{H^2\hookrightarrow L^\infty}\|\theta-\hat{\theta}\|_{L^2(\Omega)}\|\Delta\dot{\hat{\utransf}}\|_{L^2(\Omega)}\|\Delta(\dot{\utransf}-\dot{\hat{\utransf}})\|_{L^2(\Omega))}\\
&\frac{1}{2}\frac{d}{dt}\|\nabla(\dot{\utransf}-\dot{\hat{\utransf}})\|^2_{L^2(\Omega)}+(1-\rho C_{H^2\hookrightarrow L^\infty})\|\Delta(\dot{\utransf}-\dot{\hat{\utransf}})\|^2_{L^2(\Omega)}\\
&\leq \frac{1}{4\epsilon}\left(\|\hat{\theta}\|^2_{L^\infty(\Omega)}\|\dot{\utransf}-\dot{\hat{\utransf}}\|^2_{L^2(\Omega)}+C^2_{H^2\hookrightarrow L^\infty}\rho^2\|\Delta\dot{\hat{\utransf}}\|_{L^2(\Omega)}^2 \right) + \epsilon\|\Delta(\dot{\utransf}-\dot{\hat{\utransf}})\|^2_{L^2(\Omega)},
\end{align*}
where $\|\Delta\dot{\hat{\utransf}}\|_{L^2(\Omega)}$ is attained by estimating with the same technique for \eqref{transf-log-problem-1}--\eqref{transf-log-problem-3} with the coefficient $\hat{\theta}\in L^\infty(\Omega)$. Then if $\rho$ is sufficiently small and the following condition holds 
\begin{align}\label{log-cond-3}
\calX= L^p(\Omega)\hookrightarrow L^2(\Omega)\mbox{ i.e.,}\quad p\geq 2,
\end{align}
applying Gronwall's inequality then integrating on $[0,T]$ yields
\begin{equation}\label{log-positive-estimate-3}
\|\utransf-\hat{\utransf}\|_{H^1(0,T;H^2(\Omega))}\leq C\|\hat{\theta}-\theta\|_\calX\|\hat{\utransf}\|_{H^1(0,T;H^2(\Omega))} 
\end{equation}
for fixed $\hat{\utransf}=S(\hat{\theta})=S(\theta^0)$. So, $S(\calB^\calX_\rho(\theta^0))$ is bounded in $H^1(0,T;H^2(\Omega))$ and its diameter can be controlled by $\rho$. In case $d=1$, smallness of $\rho$ can be omitted if one uses the estimate \eqref{log-positive-estimate-2}.
\color{black}

\item Continuity of the inverse of the linearized model\medbreak

Now we consider the linearized problem
\begin{flalign} 
&\qquad\qquad\qquad\dot{z}(t)-\Delta z(t) + 2\nabla u(t)\cdot \nabla z(t) = r(t) \qquad t \in (0,T) & \label{log-linearized-1}\\
&\qquad\qquad\qquad z(0)=0  & \label{log-linearized-2}	
\end{flalign}
whose adjoint problem after transforming $t=T-\tau$ is
\begin{flalign} 
&\qquad\qquad\qquad\dot{p}(t)-\Delta p(t) - 2\nabla\cdot \left(\nabla u(t) p(t)\right) = \phi(t) \qquad t \in (0,T) & \label{log-adjoint-1}\\
&\qquad\qquad\qquad p(0)=0 . \label{log-adjoint-2}& 	
\end{flalign}
Since $u\in C^1(0,T;H^2(\Omega)\cap H_0^1(\Omega))$ as proven in \ref{R2}, this equation with the coefficients $m:=-2\nabla u\in C^1(0,T;H^1(\Omega)), n:=-2\Delta u\in C^1(0,T;L^2(\Omega))$ is smooth enough to attain the estimate \ref{R3} by the contraction argument.


\quad Indeed, let us take $p$ solving (\ref{log-adjoint-1})--(\ref{log-adjoint-2}), 
\\
\textcolor{green}{please mention what $\hat{u}$ is }
\\
then
\begin{flalign*}
\qquad \dot{p} &-\Delta p+\hat{m}\cdot\nabla p+\hat{n}p =\phi+ (\hat{m}-m)\cdot\nabla p+(\hat{n}-n)p&\\
\qquad p &= \left(\frac{d}{dt}-\Delta + \hat{m}\cdot\nabla+\hat{n}\right)^{-1}\left[\phi+(\hat{m}-m)\cdot\nabla p+(\hat{n}-n)p\right]&\\
&=: Tp,&
\end{flalign*}
with some $\hat{m}\in L^\infty((0,T)\times\Omega)$ and some $\hat{n}\in L^\infty((0,T)\times\Omega)$. Then for $d\leq 3$, $T: L^2(0,T;H^2(\Omega)\cap H_0^1(\Omega)) \rightarrow L^2(0,T;H^2(\Omega)\cap H_0^1(\Omega))$
is a contraction
\begin{align} \label{log-contraction}
&\|T(p - q) \|_{L^2(0,T; H^2\cap H_0^1)} \nonumber\\
&\leq \left\|\left(\frac{d}{dt}-\Delta + \hat{m}\cdot\nabla+\hat{n}\right)^{-1}\right\|_{L^2(0,T;L^2(\Omega))\rightarrow L^2(0,T;H^2\cap H_0^1)}\nonumber\\
&\qquad .\left(\|(\hat{m}-m)\cdot\nabla(p-q)\|_{L^2(0,T;L^2(\Omega))}+\|(\hat{n}-n)(p-q)\|_{L^2(0,T;L^2(\Omega))} \right)\nonumber\\
&\leq C^{\hat{\theta}} \left(\|\hat{m}-m\|_{L^\infty(0,T;H^1(\Omega))}\|\nabla(p-q)\|_{L^2(0,T;H^1(\Omega))}+\|\hat{n}-n\|_{L^\infty(0,T;L^2(\Omega))}\|p-q\|_{L^2(0,T;L^\infty(\Omega))} \right)\nonumber\\
&\leq C\epsilon \|p-q\|_{L^2(0,T;H^2\cap H_0^1)} 
\end{align}
\textcolor{green}{After the second inequality, not both norms in $\|\hat{m}-m\|_{L^\infty(0,T;L^2(\Omega))}\|\nabla(u-v)\|_{L^2(0,T;L^2(\Omega))}$ can be taken $L^2$ with respect to space. If you want to stay with $L^\infty(0,T;L^2(\Omega))$ smallness of $\hat{m}-m$ then higher regularity of $u-v$ will be needed.}\textcolor{blue}{ $\rightarrow$ fixed typo above}
\\
where $H_0^1(\Omega)\hookrightarrow L^6(\Omega), H^2(\Omega)\cap H_0^1(\Omega)\hookrightarrow L^\infty(\Omega)$ for $d\leq 3$. Above, we apply from \cite[Section 7.1.3 , Theorem 5]{Evans} the continuity of $\left(\frac{d}{dt}-\Delta + \hat{m}\cdot\nabla+\hat{n}\right)^{-1}$ with noting that, although the theorem is stated for time-independent coefficients, the proof reveals it is still applicable for $\hat{m}=\hat{m}(t,x), \hat{n}=\hat{n}(t,x)$ being bounded in time and space.\\
\color{blue}
The above constant $C^{\hat{\theta}}$, which depends on $\hat{m}\in \nabla\cdot S(\calB^\calX_\rho(\theta^0))\cap L^\infty(0,T;L^\infty(\Omega)), \hat{n}\in \Delta S(\calB^\calX_\rho(\theta^0))\cap L^\infty(0,T;L^\infty(\Omega))$ can be bounded by some constant $C$ depending only on $S(\theta^0)$ and the diameter of $S(\calB^\calX_\rho(\theta^0))$ similarly to the c-problem and a-problem if choosing $\hat{\theta}=\theta^0$. In order to make $C\epsilon$ less than one, we require $\|\hat{m}-m\|_{L^\infty(0,T;H^1(\Omega))}$ and $\|\hat{n}-n\|_{L^\infty(0,T;L^2(\Omega))}$ to be sufficiently small. Those conditions turn out to be uniform boundedness of $\|\hat{\utransf}-\utransf\|_{L^\infty(0,T;H^2(\Omega))}$ (or the diameter of $S(\calB^\calX_\rho(\theta^0))$, which can be seen as smallness of $\rho$ as in \eqref{log-positive-estimate-3} since $H^1(0,T)\hookrightarrow L^\infty(0,T)$. 
\color{black}
From that, existence of the dual state $p\in L^2(0,T; H^2(\Omega)\cap H_0^1(\Omega))$ for given $\phi\in L^2(0,T;L^2(\Omega))$ is shown.


\quad Then \ref{R3-dual} follows without adding more constraints on $p$
\begin{align*}
 \|p\|_{L^2(0,T;H^2(\Omega))}
&\leq C (\|(\hat{m}-m)\cdot\nabla p\|_{L^2(0,T;L^2(\Omega))}+\|(\hat{n}-n)p\|_{L^2(0,T;L^2(\Omega))} + \|\phi\|
_{L^2(0,T;L^2(\Omega))} ) \qquad\qquad\qquad\qquad\qquad\\\
&\leq C\|\phi\|_{L^2(0,T;L^2(\Omega))}
\end{align*}
with constant $C$ depending only on some fixed $\hat{m}, \hat{n}$ and the assumption on smallness of $\rho$.
Here with the $L^2$-norm on the right hand side, the maximum $q$ is limited by $\bar{q}=2$.\\
\hphantom{lll}Observing that the problem (\ref{log-adjoint-1})--(\ref{log-adjoint-2}) has the form of the a-problem, written in (\ref{a-rho-1}), with $\underline{a}=1, \nabla a=-2\nabla u(t) \in L^6(\Omega)$ and the additional term on the right hand side, namely,
\begin{align}
\frac{1}{2}\|np\|^2_{L^2(\Omega)}=\|\Delta up\|^2_{L^2(\Omega)}\leq \|\Delta u\|^2_{L^2(\Omega)}\|p\|^2_{L^\infty(\Omega)}\leq C^2_{H_0^1\rightarrow L^\infty}\|\Delta u\|^2_{L^2(\Omega)}\|\nabla p\|^2_{L^2(\Omega)},\label{log-rho-1}
\end{align}
if the dimension $d=1$.\\
The solution $u=S(\theta)$ also lies in some ball in $C^1(0,T;H^2(\Omega)\cap H^1_0(\Omega))$ for all $\theta\in\calB^\calX_\rho(\theta^0)$, as in \ref{R2} we have shown boundedness of the operator $S$.\\
It allows us to evaluate analogously to (\ref{a-rho-1})--(\ref{a-rho-2}) with taking into account the additional term (\ref{log-rho-1}) to eventually get
\begin{align*}
\|\Delta p\|_{L^2(0,T;L^2(\Omega))}\leq C \|\phi\|^2_{L^2(0,T;L^2(\Omega))} \qquad
\end{align*}
with the constant $C$ depending only on $\theta^0, \rho$. Hence, if $d=1$, $\rho$ is not required to be small.

\item all-at-once tangential cone condition \medbreak
According to \eqref{qhat}, \eqref{condPsi}  with $s=t=2$, $m=n=2$, $\hat{\gamma}=0, \rho=2$ we require
\[
\begin{aligned}
&2-\frac{d}{2}\succeq 1-\frac{d}{q^*}+\frac{d}{R}\mbox{ and }\\
& 1\leq\frac{R}{q^*}\mbox{ and } q\leq\hat{q} \mbox{ and }
2-\frac{d}{2}\succeq \max\left\{-\frac{d}{\hat{q}}\,, \ 1-\frac{d}{R}\right\}
\end{aligned}
\]
where the latter conditions come from the requirements $V=H^2(\Omega)\cap H_0^1(\Omega)\hookrightarrow W^{1,R}(\Omega)$.
\end{enumerate}

\begin{corollary}
Assume $u_0\in V$, and
\begin{equation} \label{log-space}
\begin{split}
\calD(F)=\calX=L^p(\Omega),  \quad\qquad Y=L^q(\Omega),\quad\qquad &V=W=H^2(\Omega)\cap H_0^1(\Omega)\\ 
&\textcolor{blue}{p\geq2},\quad q\in\left[\underline{q},2\right],\quad d\leq 3.
\end{split}
\end{equation}
with $\underline{q}=\min\limits_q \left\{ 2-\frac{d}{2}\succeq 1-d+\frac{d}{q}+\frac{d}{\check{p}} \wedge q\geq 1+\frac{1}{\check{p}-1} \right\}$.


Then $F$ satisfies the tangential cone condition (\ref{TCC-Re}) with a uniformly bounded operator $F'(\theta)$ defined by (\ref{F'}).
\end{corollary}\bigbreak

For achieving a Hilbert space setting for $X$ and $Y$, one can choose $p=q=2$ if $d\textcolor{blue}{\leq 3}$,
see also \cite{Nguyen}.


